Embedded Pattern Matching

Haskell is a popular choice for hosting deeply embedded languages. A recurring challenge for these embeddings is how to seamlessly integrate user defined algebraic data types. In particular, one important, convenient, and expressive feature for creating and inspecting data -- pattern matching -- is not directly available on embedded terms. We present a novel technique, embedded pattern matching, which enables a natural and user friendly embedding of user defined algebraic data types into the embedded language, and allows programmers to pattern match on terms in the embedded language in much the same way they would in the host language.

==> figures/llvm_quad.tex <==
% vim: syntax=tex

\begin{figure}[t]
\begin{lstlisting}[style=llvm]
  %2 = getelementptr inbounds i8, i8* %tags, i64 %1
  %3 = load i8, i8* %2                    ; read TAG value
  br label %switch.entry                  ; branch to switch statement

switch.entry:
  switch i8 %3, label %switch.default [   ; jump table
    i8 0, label %switch.l0                ; A
    i8 2, label %switch.l2                ; B
    i8 1, label %switch.l1                ; C
    i8 3, label %switch.l3                ; D
  ]

switch.l0:                               ; code to execute for `A' constructor
  |\ldots|
\end{lstlisting}
\caption{Representative LLVM code generated for embedded \lstinline[style=inline]{case} expressions}
\label{fig:llvm_quad}
\end{figure}



==> section/future.tex <==
\section{Future Work}
\label{sec:future}

% \paragraph{Recursive data types:}
% \label{sec:recursive_types}
%
% Our solution to pattern matching works for arbitrarily nested sum and
% product data types, but not for \emph{recursive} data
% types, such as lists or trees. While recursive types are an important feature for most stand-alone
% functional languages, in the context of deeply embedded languages they
% are an esoteric feature not found in any embedded language we know of.


\paragraph{Compact representation of sum data types:}
\label{sec:compact_sums}

As we described in Section~\ref{sec:sum_types}, our representation reserves
memory for all of the fields for every constructor of a sum type. This
is safe, as our embedded pattern synonyms prevent access to any undefined values,
but memory inefficient, especially for data types with many (non-nullary)
constructors and/or constructors with many fields. While a memory efficient
representation is desirable, it is orthogonal to our contribution.

% Futhark~\cite{Henriksen:2017}, a standalone language for data-parallel arrays
% similar in spirit to Accelerate, uses the same memory-inefficient layout of
% data.

\paragraph{Type-safe constructor tags:}
\label{sec:sop_typed_tags}

Similarly, there is no connection between the integer tag we use to distinguish
constructor alternatives, and the fields associated with that constructor
containing valid data. One solution is to take inspiration from the
sum-of-products style of generic programming~\cite{deVries:2014} and lift the
integer tag to a type-level natural number, which is used to provide a
type-level lookup to the types of the valid field projections. This would
provide certainty that undefined values are never accessed, but is again
orthogonal to this work.


\paragraph{Literal patterns:}
\label{sec:literal_patterns}

Pattern matching in Haskell supports several use cases beyond matching on
algebraic data types, and it would be desirable to support these features in
embedded pattern matching as well. For example, instead of using a regular
@if-then-else@ construct we might like to write the following:
%
\begin{haskell}
isZero :: %\textcolor{exp}{Exp Int}% -> %\textcolor{exp}{Exp Bool}%
isZero 0 = True_
isZero _ = False_
\end{haskell}
%
Unfortunately, the Haskell compiler currently desugars pattern matches of this
form into a program which does not type check. % , and compilation
                                % fails
%
% %
% During compilation of the host program the Haskell compiler will desugar this
% into a program into the following form:
% %
% \begin{haskell}
% isZero x =
%   case x == fromInteger 0 of
%     True  -> True_
%     False -> False_
% \end{haskell}
% %
% This program does not type check, and thus compilation fails. Our equality
% operator on embedded terms @(==)@ returns an @Exp Bool@ result, but the
% desugared program matches directly against a regular @Bool@.
% % \tlm{we could drop this detailed explanation and just say it is desugared into a
% % form that doesn't typecheck before we get a chance to do something about it}
%
% In future it might be possible to overcome this limitation,
% to add support for pattern matching on numeric literals,
Future work may overcome this limitation,
but for now we chose to focus on pattern matching on algebraic
data types, for which embedded languages previously had no alternative.


% \tlm{This is maybe less relevant for the more-general ESOP audience}
% \TODO{make this more general; the main focus/feature of this work is pattern
% matching on algebraic data types. pattern matching in haskell also supports
% other features that we don't yet, such as ... it may be interesting to
% investigate those in futer work. at least for literals there is an easy
% alternative with ifThenElse, but that was not the case for ADTs}
%
% Pattern matching is a convenient way to inspect the constructors of a data type,
% and this work has shown how to extend this to pattern matching on embedded
% language terms. However, Haskell also allows overloaded numeric literals in
% patterns, and it would be desirable to also support this feature in embedded
% pattern matching. For example, we may like to write the following embedded term:
% %
% \begin{haskell}
% isZero :: Num a => Exp a -> Exp Bool
% isZero 0 = True_
% isZero _ = False_
% \end{haskell}
% %
% During the host program compilation, GHC will desugar this program into:
% %
% \begin{haskell}
% isZero x =
%   case x == fromInteger 0 of
%     False -> False_
%     True  -> True_
% \end{haskell}
% %
% And at this point we are stuck. We cannot overload the @Eq@ class to operate on
% embedded terms, as the types of those operations are fixed to returning a
% regular Haskell Boolean. We can use the Rebindable Syntax extension so that our
% equality operator on embedded terms is used instead of the definition from the
% type's @Eq@ instance, namely:
% %
% \begin{haskell}
% (==) :: Eq a => Exp a -> Exp a -> Exp Bool
% \end{haskell}
% %
% but this causes the desugared program to fail type-checking, and thus host
% program compilation fails. The pattern cases match against Boolean values @True@
% and @False@, but our equality operator returns an \emph{embedded} Boolean. These
% problems currently stand in the way of supporting literal patterns in languages
% embedded in Haskell. A different host language may not encounter this issue, but
% investigating this is outside the scope of this work.



==> section/scala.tex <==
\section{Applicability to other languages}
\label{sec:other_languages}

In this paper, we focus on the implementation of our technique in Haskell, and
we made use of several Haskell language extensions to do so. Pattern synonyms
allow us to give pattern matching on embedded algebraic data types the look and
feel of pattern matching in the host language, but are not required for the core
technique, which is the @match@ function to explore the alternatives of a @case@
expression, together with the builder and matcher functions for each constructor.
GADTs and type families are used to maintain an intrinsically typed abstract
syntax tree, but are unnecessary with a uni-typed AST defined as a regular sum
data type. The internal representation of user defined abstract data types and
computations, which we propose in this paper, does not require any special host
language features.

To demonstrate how our technique carries over to a different, but similarity
expressive language, we also implemented embedded pattern matching in Scala.
%
Owing to the fact that Scala is at its core an object oriented
language, the implementation is, of course, structured
differently. The main technical change is in the mapping between the
source and representation types, which is done via implicits in the
Scala implementation whereas the Haskell implementation uses associated
types. As implicits are not unique, we have to witness the @Exp@
constructor on both the surface as well as the representation type.
This results in relatively verbose code, but this could be addressed by using
type synonyms to refer to the representation type. Another minor difference
is the way @match@ (renamed @caseof@ as that keyword is already taken) is
overloaded to accept functions of different arity. Apart from these
considerations, the embedded pattern matching implementation as described in
this paper is translated to Scala in a straightforward way.
The code for this implementation is also available at \emph{redacted for review}.

% For example, the projection in @matchJust@ requires a certain structure to the
% representation (which the implementation of course uses), but the compiler can't
% prove that it will be the only implementation that will exist - or that it will
% be using this implementation if there's multiple ones.

% To make this a bit less verbose, we can define a type synonym to talk about the
% representation type, but it has to be just a simple type synonym - not a type
% family or associated type. This is because, even though types can be defined on
% Scala implicit instances (a form of associated types), implicits are passed
% \emph{after} the regular arguments, and those arguments can't be referenced in
% earlier argument lists. For example, the following doesn't work for that reason:

% \begin{lstlisting}
% trait Elt[A] {
%   type Repr
% }

% //                          | cannot reference elt here
% case class Exp[A](x: PreExp[elt.Repr])(implicit elt: Elt[A])
% \end{lstlisting}

% I suspect that allowing these back-references wouldn't be enough to write the
% implementation word-for-word like Haskell, since we still have the problem of
% wanting to project onto an unknown representation later on. In a Haskell where
% we allowed multiple typeclass implementations, we might try to add an equality
% contraint based on the instance stored in the GADT (i.e. @Elt a => Const :: a -> PreExp a@),
% but even then it seems like it would require a runtime check on which instance
% is in use, so this equality constraint wouldn't work without something like
% Haskell's @Typeable@ reflection. Scala has a way of talking about equality
% constraints which I haven't had much success with (@=:=@), and I haven't found
% an equivalent to @Just Refl@, since @Refl@ would equivalently be a constructor
% of @=:=@ in Haskell, but in Scala this type is abstract.


% It's simpler (not sure if required) to use the @Exp@/@PreExp@ combination here
% because it allows us to witness the @PreExp@ type on only the representation. We
% could potentially do away with the wrapper and just put both the type variables
% on the @PreExp@ type, but then we have weird situations where we have to have a
% pair in the representation and surface types of the @Pair@ constructor - which
% is of course correct but then we'd need an additional constructor (e.g. @Tuple@)
% to "cast" that surface type to another surface type that's represented by that
% pair structure, and that @Tuple@ constructor would have less use compared to the
% @Exp@ constructor, because the @Exp@ constructor also stores the @Elt@ implicit
% for the type, which means functions don't have to include that in their
% contexts.

% Our @caseof@ (@match@ is a keyword in Scala) function accepts uncurried
% functions, and just has multiple overloaded implementations for multiple lengths
% of argument lists. Scala does have a way to, curry and uncurry any function, but
% we require the implicit @Elt@ for the output type to be in context, which would
% get in the way of the recursion. Additionally, this implicit also needs to be
% passed in the use site:

% \begin{lstlisting}
% //           | this implicit can't be skipped over before applying the returned function
% caseof(go _)(eltInt)(x)
% \end{lstlisting}


